Empirical Analysis of Model Selection for Heterogeneous Causal Effect Estimation

We study the problem of model selection in causal inference, specifically for conditional average treatment effect (CATE) estimation. Unlike machine learning, there is no perfect analogue of cross-validation for model selection as we do not observe the counterfactual potential outcomes. Towards this, a variety of surrogate metrics have been proposed for CATE model selection that use only observed data. However, we do not have a good understanding regarding their effectiveness due to limited comparisons in prior studies. We conduct an extensive empirical analysis to benchmark the surrogate model selection metrics introduced in the literature, as well as the novel ones introduced in this work. We ensure a fair comparison by tuning the hyperparameters associated with these metrics via AutoML, and provide more detailed trends by incorporating realistic datasets via generative modeling. Our analysis suggests novel model selection strategies based on careful hyperparameter selection of CATE estimators and causal ensembling.

==> comments.tex <==
**Important**  
- We will motivate the two-level model selection strategy as being inspired from the congeniality bias; that is why we should use the appropriate metrics conditioned on a particular type of Meta Learner.
- The definition of congeniality bias is different in Curth et al. work; and we should adopt the same as well.
- We need to convert things into plots and huge tables should be presented in appendix.

The focus will be changed a lot from finding the optimal metric to the right design choice for model selection, mentioned explicitly in introduction and the way results are presented. There will be a few lines at the end stating that some metrics do perform better than the other, when we talk about comparing the performance of our proposed scores as well.

\begin{itemize}
    \item We will highlight the overall design of our model selection strategy first and then talk about the details of various estimators and metrics.
    \begin{itemize}
        \item Work on a figure for the overall design; which incorporates two level and causal ensembling as well
        \item Add a figure explaining the difference between single level and two level selection strategy
        \item Add a figure explaining ensembling
    \end{itemize}
    \item Frame specific research questions in the experiment sections so that it appears you put more thought into; the research questions are basically does hyperparameter tuning leads to differences. Then ensembling, new scores as they are also the contribution of our work. And congeniality bias as it was studied by Curth et al.    \item Mention why we did not use Mu Score (Factual Prediction criteria) as not all CATE estimators can be evaluated using that.
    
    \item AutoML part in our pipeline should be highlighted in experiments separately, and whether it already leads to SOTA results w.r.t CATE estimators themselves.
    \item The point in section 4 of Curth et al. about caring about the performance of estimators is something that I should focus on as well. Basically add a table atleast for different Meta Learners and the performance they obtain across various datasets.
    \item We need to explicitly mention results about congeniality bias of plug in and indirect metrics as that was one major takeway of Curth et al.
    \item A clear related works section at the end where we again show why our design choice is different from prior works.


- Point in the appendix something like an improvement table and specifically mention that some metrics struggle a lot with getting the hyperparameters of meta-learners correct. This makes it feel that we are doing a better job at understanding the flaws with different metrics.
    
\end{itemize}
